ARMS: A Vision for Actor Reputation Metric Systems in the Open-Source Software Supply Chain

Many critical information technology and cyber-physical systems rely on a supply chain of open-source software projects. OSS project maintainers often integrate contributions from external actors. While maintainers can assess the correctness of a pull request, assessing a pull request's cybersecurity implications is challenging. To help maintainers make this decision, we propose that the open-source ecosystem should incorporate Actor Reputation Metrics (ARMS). This capability would enable OSS maintainers to assess a prospective contributor's cybersecurity reputation. To support the future instantiation of ARMS, we identify seven generic security signals from industry standards; map concrete metrics from prior work and available security tools, describe study designs to refine and assess the utility of ARMS, and finally weigh its pros and cons.

==> table.tex <==
%&ignore
{
% [placeholder: data in table \ref{tab:evaluation_metrics}]
% p{0.32\linewidth}
% \begin{table*}
%     \centering
%     \caption{Proposed Signal Evaluation Method}
%     \label{tab:benchmark_comparison}
%     \small
%     \begin{tabular}{|l|l|l|l|}
%         \hline
%         \textbf{Proposed Security Signal }& \textbf{Description} & \textbf{Analysis Metrics}  & \textbf{Description} \\
%         \hline
%         \multirow{3}{*}{\textbf{Security vulnerability in artifact -- Pull Requests/Commits }} & L         & XXX & XXX  \\
%                                              & T  & XXX & XXX \\
%                                              & E & XXX & XXX \\
%         \hline
%         \multirow{3}{*}{\textbf{Security vulnerability in artifact -- use of vulnerable dependencies}} & L (ms)          & XXX & XXX \\
%                                              & T   & XXX & XXX \\
%                                              & E & XXX & XXX \\
%         \hline
%         \multirow{3}{*}{\textbf{Use of ecosystem code scanning and security analysis features}} & L         & XXX & XXX\\
%                                              & T  & XXX & XXX \\
%                                              & E & XXX & XXX \\
%         \hline
%         \multirow{3}{*}{\textbf{use of ecosystem integrity guarantees}} & L          & XXX & XXX \\
%                                              & T  & XXX & XXX \\
%                                              & E & XXX & XXX  \\
%         \hline
%         \multirow{3}{*}{\textbf{Use of branch protection}} & L        & XXX & XXX \\
%                                              & T  & XXX & XXX  \\
%                                              & E & XXX & XXX  \\
%         \hline
%         \multirow{3}{*}{\textbf{Security policies and vulnerability reporting}} & L          & XXX & XXX \\
%                                              & T  & XXX & XXX \\
%                                              & E & XXX & XXX  \\
%         \hline
%         \multirow{3}{*}{\textbf{Workflow automation}} & L        & XXX & XXX \\
%                                              & T  & XXX & XXX  \\
%                                              & E & XXX & XXX  \\
%         \hline
%     \end{tabular}
% \end{table*}
% \begin{table*}
%     \centering
%     \caption{Proposed Signal Evaluation Method}
%     \label{tab:benchmark_comparison}
%     \scriptsize
%     \begin{tabular}{|l|p{0.4\linewidth}|l|}
%         \hline
%         \textbf{Proposed Security Signal} & \textbf{Description} & \textbf{Analysis Metrics} \\
%         \hline
%         \multirow{3}{*}{\textbf{Security vulnerability in artifact -- Pull Requests/Commits}} 
%                                              & Measures the presence of vulnerabilities introduced via pull requests or commits. It is recommended that vulnerabilities be fixed as early as possible. \\
%                                              % Explanation of the latency metric (L), which measures the time taken to detect vulnerabilities in pull requests.Explanation of the efficiency metric (E), which evaluates the overall efficiency of security checks on pull requests.Explanation of the throughput metric (T), which assesses the number of vulnerable commits handled per time unit \\
%                                              & & Average time in fixing security vulnerability (measured by severity levels)  \\
%                                              & & T   \\
%                                              & & E  \\
%         \hline
%         \multirow{3}{*}{\textbf{Security vulnerability in artifact -- use of vulnerable dependencies}} 
%                                              & Assesses if vulnerable dependencies are being introduced into the artifact.Efficiency metric (E) description for the effectiveness of dependency vulnerability scans.Throughput metric (T) description for how many dependencies are checked per unit of time. Latency metric (L) description for dependency vulnerability checks \\
%                                              & & L   \\
%                                              & & T  \\
%                                              & & E \\
%         \hline
%         \multirow{3}{*}{\textbf{Use of ecosystem code scanning and security analysis features}} 
%                                              & Evaluates whether the ecosystem's security tools are being used for code scanning 
%                                              & L   \\
%                                              & & T  \\
%                                              & & E \\
%                                              % & L         & Latency metric (L) description for the time it takes to scan the code \\
%                                              % & & T  & Throughput metric (T) description for the number of scans done over time \\
%                                              % & & E & Efficiency metric (E) description for the effectiveness of the scanning tools used \\
%         \hline
%         \multirow{3}{*}{\textbf{Use of ecosystem integrity guarantees}} 
%                                              & Examines whether ecosystem guarantees for integrity (e.g., code signing) are used  
%                                              & L   \\
%                                              & & T  \\
%                                              & & E \\
%                                              % & Latency metric (L) description for the time taken to apply integrity checks \\
%                                              % & & T  & Throughput metric (T) description for the number of integrity verifications over time \\
%                                              % & & E & Efficiency metric (E) description for the effectiveness of ecosystem integrity tools \\
%         \hline
%         \multirow{3}{*}{\textbf{Use of branch protection}} 
%                                              & Checks if branch protection measures are in place to prevent unauthorized changes 
%                                              & L   \\
%                                              & & T  \\
%                                              & & E \\
%                                              % & L        & Latency metric (L) description for how fast branch protection is enforced \\
%                                              % & & T  & Throughput metric (T) description for the number of branch protections applied over time \\
%                                              % & & E & Efficiency metric (E) description for the robustness of branch protection mechanisms \\
%         \hline
%         \multirow{3}{*}{\textbf{Security policies and vulnerability reporting}} 
%                                              & Determines if the project has defined security policies and vulnerability reporting mechanisms
%                                              & L   \\
%                                              & & T  \\
%                                              & & E \\
%                                              % & L          & Latency metric (L) description for reporting vulnerabilities \\
%                                              % & & T  & Throughput metric (T) description for the number of policies or reports handled \\
%                                              % & & E & Efficiency metric (E) description for the clarity and actionability of security policies \\
%         \hline
%         \multirow{3}{*}{\textbf{Workflow automation}} 
%                                              & Assesses the use of automation in workflows to enforce security practices 
%                                              & L   \\
%                                              & & T  \\
%                                              & & E \\
%                                              % & L        & Latency metric (L) description for how quickly workflows are automated for security \\
%                                              % & & T  & Throughput metric (T) description for the number of automated workflows executed \\
%                                              % & & E & Efficiency metric (E) description for the effectiveness of automated security workflows \\
%         \hline
%     \end{tabular}
% % \end{table*}
% {
% 	%\arraystretch{1.5}
% 	\begin{table*}[!t]
% 		\centering
% 		\caption{
% 			Proposed Signal Evaluation Method. We have categorized proposed security signals, and their descriptions and metrics are provided for evaluation purposes.
% 		}
% 		\normalsize
% 		\small
%         \scriptsize
% 		\begin{tabular}{p{0.05\linewidth}p{0.37\linewidth}p{0.4\linewidth}}
%             \toprule
%            \textbf{Signal No.} &\textbf{Proposed Security Signal \& Analysis Metrics} & \textbf{Description} \\
%             \toprule
%         \textbf{1.} & \textbf{Security vulnerability in artifact -- Pull Requests/Commits} & Measures vulnerabilities introduced through pull requests or commits. Introduced either by the user, or to a project owned by the user. \\
%         a. & Average time in fixing/closing security vulnerability of various severity levels & {}\\
%          b. & Severity levels of security vulnerability reported. & {}\\
%           c. & Presence of vulnerability in PR/commits (not linked to external dependencies) & {} \\
%         % & L  & Time taken to detect vulnerabilities in pull requests \\
%         % &  & T  & Number of vulnerable commits processed over time \\
%         % &  & E & Efficiency of security checks on pull requests \\
%         \midrule
%         \textbf{2.} & \textbf{Security vulnerability in artifact -- use of vulnerable dependencies} & Assesses if vulnerable dependencies are introduced into the artifact\\
%         a. & Average length of time before fix & {} \\
%         b. & Severity levels of package’s reported vulnerability & {}  \\
%         c. &  Number of Repos/Projects that has a vulnerable dependency .& {} \\
%         d. & Average number of vulnerable dependencies/project. & {}  \\
%         e. & Average number of projects with reported vulnerable dependencies& {} \\
%         % & L  & Latency in detecting dependency vulnerabilities \\
%         % &  & T  & Number of dependencies checked over time \\
%         % &  & E & Efficiency of scanning vulnerable dependencies \\
%         \midrule
%         \textbf{3.} & \textbf{Use of ecosystem code scanning and security analysis features} & Evaluates usage of ecosystem's security tools for code scanning\\
%         a. & Status of dependabot alerts (for dependencies) & {}  \\
%          b. &  Status of Secret sharing/Validity Checks. & {}  \\
%          c. &  Code scanning and Vulnerability alerts & {}  \\ 
%        d. &  Push Protection Status & {} \\
%         % & L  & Time to complete a code scan \\
%         % &  & T  & Number of scans performed per time unit \\
%         % &  & E & Effectiveness of scanning tools \\
%         \midrule
%         \textbf{4.} & \textbf{Use of ecosystem integrity guarantees} & Examines use of ecosystem integrity features (e.g., code signing) \\
%          a. & Average Number of Projects with an integrity guarantee. & {}  \\
%          % L & {} & {} \\
%          %  L & {} & {} \\
%         % & L  & Time to apply integrity checks \\
%         % &  & T  & Number of integrity verifications done over time \\
%         % &  & E & Effectiveness of integrity tools \\
%         \midrule
%        \textbf{5.} & \textbf{Use of branch protection} & Checks if branch protection is enforced to prevent unauthorized changes\\
%          a. & Average Number of protected branch per project & {} \\
%          b. & Number of Projects with Protected branch  & {}\\
%           % L & {} & {} \\
%         % & L  & Time taken to apply branch protection \\
%         % &  & T  & Number of branches protected per unit of time \\
%         % &  & E & Efficiency of branch protection mechanisms \\
%         \midrule
%         \textbf{6.} & \textbf{Use of security policies and vulnerability reporting} & Determines if project has security policies and reporting mechanisms\\
%          a. & status of private vulnerability reporting, or security policy & {} \\
%          % L & {} & {} \\
%          %  L & {} & {} \\
%         % & L  & Time taken to report vulnerabilities \\
%         % &  & T  & Number of policies or reports handled \\
%         % &  & E & Clarity and effectiveness of security policies \\
%         \midrule
%         \textbf{7.} & \textbf{Use of automated workflows} & Assesses use of automation in workflows to enforce security.\\
%         a. & Average Number of Projects with Automated workflow & {}\\
%          % L & {} & {} \\
%          %  L & {} & {} \\
%         \bottomrule
% 		\end{tabular}
% 		\label{tab:signal_evaluation}
% 	\end{table*}
% }
%\arraystretch{1.5}
% \KC{TODOS;
% 1. Intro and background
% 2. add disclaimers for what work did and did not do.
% 3. Table caption and refs
% }
\begin{table*}[!t]
\centering
\caption{
    % Proposed security metrics and evaluation methods. Metric categories in bolded fonts are derived from recommendations from security recommendations from NIST, SLSA, and CNCF. Sub-metrics provide means of evaluating the proposed metrics. We also cite potential security case study that warrants inclusion of these metrics.
    % Proposed security Signals, weightage signals, and evaluation metrics. Bolded security and weightage signals are derived from security recommendations \eg NIST, SLSA, CNCF, etc, and previous works respectively. The proposed metrics offer ways to evaluate the highlighted security signal. Relevant security case studies and (or) related works are cited to justify the inclusion of these metrics.
    Proposed security signals, weighting factors, and evaluation metrics. Bolded security and weighting signals are derived from established frameworks (e.g., NIST, SLSA, CNCF) and prior work, respectively. The proposed metrics describe how to measure each highlighted security or weighting signal. Relevant case studies and related research are cited to justify inclusion of select metrics.
    % We have categorized proposed security signals, and their descriptions and metrics are provided for evaluation purposes.
}
\normalsize
\small
\scriptsize
\begin{tabular}{p{0.01\linewidth}p{0.37\linewidth}p{0.520\linewidth}}
% p{0.13\linewidth}
% \textbf{Potential Case Study Use}
    \toprule
   \textbf{S/N.} &\textbf{Proposed Signals \& Analysis Metrics} & \textbf{Description} \\
\toprule
\textbf{} & \textbf{\textit{\ul{SECURITY SIGNALS}}} &  \\
%\hdashline[1.5pt/5pt]
 {} & {} & {} \\

\textbf{1.} & \textbf{Security vulnerability in artifact -- Pull Requests/Commits} & Measures vulnerabilities introduced through pull requests or commits. Introduced either by the user or to a project owned by the user. \\
%\hdashline[1.5pt/5pt]
a. & Time to fix/close security vulnerabilities of various severity levels~\cite{boughton_decomposing_2024}& Time taken to address vulnerabilities detected in pull requests or commits.\\
%\hdashline[1.5pt/5pt]
b. & Severity levels of security vulnerability reported~\cite{shukla_vulnerability_detection} & Evaluates the criticality of reported vulnerabilities (low, medium, high), for user's projects.\\
%\hdashline[1.5pt/5pt]
c. & Presence of vulnerability in PR/commits (not linked to external dependencies)~\cite{gonzalez_anomalicious_2021} & Measures severity of vulnerabilities that stem from user's direct contributions. \\
% d. & Presence of vulnerability in PR/commits (not linked to external dependencies) & Measures whether vulnerabilities stem from direct contributions rather than external sources. \\
\midrule
\textbf{2.} & \textbf{Security vulnerability in artifact -- use of vulnerable dependencies} & Assesses the use and introduction of vulnerable dependencies into the artifact. \\
%\hdashline[1.5pt/5pt]
a. & Length of time before fix~\cite{boughton_decomposing_2024} & Time taken to resolve vulnerable dependencies, after they have been detected (or publicized).\\
%\hdashline[1.5pt/5pt]
b. & Severity levels of package’s reported vulnerability~\cite{shukla_vulnerability_detection} & Tracks severity of vulnerabilities in dependencies.\\
%\hdashline[1.5pt/5pt]
c. & Number of Repos/Projects that have a vulnerable dependency & Total number of projects affected by vulnerable dependencies as a percentage of users total projects.\\
%\hdashline[1.5pt/5pt]
d. & Number of vulnerable dependencies/project & Assesses how widespread vulnerable dependencies are within each project. \\
%\hdashline[1.5pt/5pt]
e. & Number of projects with reported vulnerable dependencies & Measures the overall exposure of projects to vulnerable dependencies. \\
\midrule
\textbf{3.} & \textbf{Use of ecosystem code scanning and security analysis features} & Evaluates usage of ecosystem's security tools for code scanning. \\
% & Potentially stops the use of exposed user secrets ~\cref{colonial pipeline} 
%\hdashline[1.5pt/5pt]
a. & Status of dependabot alerts (for dependencies)\cite{fischer2023effectiveness} & Monitors if security alerts for dependencies are being addressed.\\
%\hdashline[1.5pt/5pt]
b. & Status of Secret sharing/Validity Checks & Evaluates the management of secret-sharing mechanisms and validity checks.\\
%\hdashline[1.5pt/5pt]
c. & Code scanning and Vulnerability alerts\cite{fischer2023effectiveness} & Assesses if security scanning tools are actively used and vulnerability alerts managed. \\ 
%\hdashline[1.5pt/5pt]
d. & Push Protection Status & Checks if protection features are used to block pushes with exposed secrets (e.g., unscanned code). \\
\midrule
\textbf{4.} & \textbf{Use of ecosystem integrity guarantees} & Examines use of ecosystem integrity features (e.g., code signing). \\
%\hdashline[1.5pt/5pt]
a. & Number of Projects with an integrity guarantee~\cite{schorlemmer_signing_2024} & Measures how many projects are secured with integrity verification features such as code signing. \\
\midrule
\textbf{5.} & \textbf{Use of branch protection} & Checks if branch protection is enforced to prevent unauthorized changes. \\
%\hdashline[1.5pt/5pt]
a. & Number of protected branches per project & Evaluates how many branches within each project are safeguarded against direct commits. \\
%\hdashline[1.5pt/5pt]
b. & Number of Projects with Protected branches~\cite{Scorecard,zahan_openssf_2023} & Tracks how many projects enforce branch protection. \\
\midrule
\textbf{6.} & \textbf{Use of security policies and vulnerability reporting} & Determines if the project has security policies and reporting mechanisms. \\
%\hdashline[1.5pt/5pt]
a. & Status of private vulnerability reporting, or security policy~\cite{Scorecard} & Checks if private vulnerability reporting channels and security policies are established and functional. \\
\midrule
\textbf{7.} & \textbf{Use of automated workflows} & Assesses use of~\cite{Scorecard} automation in workflows to enforce security.\\
%\hdashline[1.5pt/5pt]
a. & Number of Projects with Automated workflows~\cite{Scorecard} & Measures how many user's projects use automated workflows for security enforcement, such as auto-deployments or auto-tests. \\
\midrule
\midrule
\textbf{} & \textbf{\textit{\ul{REPUTATION WEIGHTAGE SIGNALS}}} &  \\
%\hdashline[1.5pt/5pt]
 {} & {} & {} \\
% \midrule
\textbf{W1.} & \textbf{Package Usage\cite{boysel_no_nodate}} &  \\
%\hdashline[1.5pt/5pt]
 {a.} & {Number of downloads/stars/forks} & {Weighs the potential contributor's ownership of useful projects to the ecosystem.} \\
 \midrule
\textbf{W2.} & \textbf{Community Tenure \cite{boughton_decomposing_2024}} &  \\
%\hdashline[1.5pt/5pt]
 {a.} & {Length of time contributing to project } & {Weighs how much time user has been a contributor to other projects.} \\
  {b.} & {Length of time owning account} & {Weighs how long user has actually owned an account}
  \\
   {c.} & {Contributory Strength } & {Weighs the strength of contributions to other projects by lines of code, issues, pull requests}
   \\
\midrule
\textbf{W3.} & \textbf{Centrality Score\cite{hamer_trusting_2025}} &  \\
%\hdashline[1.5pt/5pt]
 {a.} & {Connections to other Actors\cite{hamer_trusting_2025}} & {Weighs a potential contributor's network of interactions/contributory activities.} \\
  {b.} & {Time to form connections} & {Length of time taken to form the connections in 'a' above.} \\
\bottomrule
\end{tabular}
\label{tab:signal_evaluation}
\end{table*}
}

==> table2.tex <==
%&ignore
{
% [placeholder: data in table \ref{tab:evaluation_metrics}]
% p{0.32\linewidth}
% \begin{table*}
%     \centering
%     \caption{Proposed Signal Evaluation Method}
%     \label{tab:benchmark_comparison}
%     \small
%     \begin{tabular}{|l|l|l|l|}
%         \hline
%         \textbf{Proposed Security Signal }& \textbf{Description} & \textbf{Analysis Metrics}  & \textbf{Description} \\
%         \hline
%         \multirow{3}{*}{\textbf{Security vulnerability in artifact -- Pull Requests/Commits }} & L         & XXX & XXX  \\
%                                              & T  & XXX & XXX \\
%                                              & E & XXX & XXX \\
%         \hline
%         \multirow{3}{*}{\textbf{Security vulnerability in artifact -- use of vulnerable dependencies}} & L (ms)          & XXX & XXX \\
%                                              & T   & XXX & XXX \\
%                                              & E & XXX & XXX \\
%         \hline
%         \multirow{3}{*}{\textbf{Use of ecosystem code scanning and security analysis features}} & L         & XXX & XXX\\
%                                              & T  & XXX & XXX \\
%                                              & E & XXX & XXX \\
%         \hline
%         \multirow{3}{*}{\textbf{use of ecosystem integrity guarantees}} & L          & XXX & XXX \\
%                                              & T  & XXX & XXX \\
%                                              & E & XXX & XXX  \\
%         \hline
%         \multirow{3}{*}{\textbf{Use of branch protection}} & L        & XXX & XXX \\
%                                              & T  & XXX & XXX  \\
%                                              & E & XXX & XXX  \\
%         \hline
%         \multirow{3}{*}{\textbf{Security policies and vulnerability reporting}} & L          & XXX & XXX \\
%                                              & T  & XXX & XXX \\
%                                              & E & XXX & XXX  \\
%         \hline
%         \multirow{3}{*}{\textbf{Workflow automation}} & L        & XXX & XXX \\
%                                              & T  & XXX & XXX  \\
%                                              & E & XXX & XXX  \\
%         \hline
%     \end{tabular}
% \end{table*}
% \begin{table*}
%     \centering
%     \caption{Proposed Signal Evaluation Method}
%     \label{tab:benchmark_comparison}
%     \scriptsize
%     \begin{tabular}{|l|p{0.4\linewidth}|l|}
%         \hline
%         \textbf{Proposed Security Signal} & \textbf{Description} & \textbf{Analysis Metrics} \\
%         \hline
%         \multirow{3}{*}{\textbf{Security vulnerability in artifact -- Pull Requests/Commits}} 
%                                              & Measures the presence of vulnerabilities introduced via pull requests or commits. It is recommended that vulnerabilities be fixed as early as possible. \\
%                                              % Explanation of the latency metric (L), which measures the time taken to detect vulnerabilities in pull requests.Explanation of the efficiency metric (E), which evaluates the overall efficiency of security checks on pull requests.Explanation of the throughput metric (T), which assesses the number of vulnerable commits handled per time unit \\
%                                              & & Average time in fixing security vulnerability (measured by severity levels)  \\
%                                              & & T   \\
%                                              & & E  \\
%         \hline
%         \multirow{3}{*}{\textbf{Security vulnerability in artifact -- use of vulnerable dependencies}} 
%                                              & Assesses if vulnerable dependencies are being introduced into the artifact.Efficiency metric (E) description for the effectiveness of dependency vulnerability scans.Throughput metric (T) description for how many dependencies are checked per unit of time. Latency metric (L) description for dependency vulnerability checks \\
%                                              & & L   \\
%                                              & & T  \\
%                                              & & E \\
%         \hline
%         \multirow{3}{*}{\textbf{Use of ecosystem code scanning and security analysis features}} 
%                                              & Evaluates whether the ecosystem's security tools are being used for code scanning 
%                                              & L   \\
%                                              & & T  \\
%                                              & & E \\
%                                              % & L         & Latency metric (L) description for the time it takes to scan the code \\
%                                              % & & T  & Throughput metric (T) description for the number of scans done over time \\
%                                              % & & E & Efficiency metric (E) description for the effectiveness of the scanning tools used \\
%         \hline
%         \multirow{3}{*}{\textbf{Use of ecosystem integrity guarantees}} 
%                                              & Examines whether ecosystem guarantees for integrity (e.g., code signing) are used  
%                                              & L   \\
%                                              & & T  \\
%                                              & & E \\
%                                              % & Latency metric (L) description for the time taken to apply integrity checks \\
%                                              % & & T  & Throughput metric (T) description for the number of integrity verifications over time \\
%                                              % & & E & Efficiency metric (E) description for the effectiveness of ecosystem integrity tools \\
%         \hline
%         \multirow{3}{*}{\textbf{Use of branch protection}} 
%                                              & Checks if branch protection measures are in place to prevent unauthorized changes 
%                                              & L   \\
%                                              & & T  \\
%                                              & & E \\
%                                              % & L        & Latency metric (L) description for how fast branch protection is enforced \\
%                                              % & & T  & Throughput metric (T) description for the number of branch protections applied over time \\
%                                              % & & E & Efficiency metric (E) description for the robustness of branch protection mechanisms \\
%         \hline
%         \multirow{3}{*}{\textbf{Security policies and vulnerability reporting}} 
%                                              & Determines if the project has defined security policies and vulnerability reporting mechanisms
%                                              & L   \\
%                                              & & T  \\
%                                              & & E \\
%                                              % & L          & Latency metric (L) description for reporting vulnerabilities \\
%                                              % & & T  & Throughput metric (T) description for the number of policies or reports handled \\
%                                              % & & E & Efficiency metric (E) description for the clarity and actionability of security policies \\
%         \hline
%         \multirow{3}{*}{\textbf{Workflow automation}} 
%                                              & Assesses the use of automation in workflows to enforce security practices 
%                                              & L   \\
%                                              & & T  \\
%                                              & & E \\
%                                              % & L        & Latency metric (L) description for how quickly workflows are automated for security \\
%                                              % & & T  & Throughput metric (T) description for the number of automated workflows executed \\
%                                              % & & E & Efficiency metric (E) description for the effectiveness of automated security workflows \\
%         \hline
%     \end{tabular}
% % \end{table*}
% {
% 	%\arraystretch{1.5}
% 	\begin{table*}[!t]
% 		\centering
% 		\caption{
% 			Proposed Signal Evaluation Method. We have categorized proposed security signals, and their descriptions and metrics are provided for evaluation purposes.
% 		}
% 		\normalsize
% 		\small
%         \scriptsize
% 		\begin{tabular}{p{0.05\linewidth}p{0.37\linewidth}p{0.4\linewidth}}
%             \toprule
%            \textbf{Signal No.} &\textbf{Proposed Security Signal \& Analysis Metrics} & \textbf{Description} \\
%             \toprule
%         \textbf{1.} & \textbf{Security vulnerability in artifact -- Pull Requests/Commits} & Measures vulnerabilities introduced through pull requests or commits. Introduced either by the user, or to a project owned by the user. \\
%         a. & Average time in fixing/closing security vulnerability of various severity levels & {}\\
%          b. & Severity levels of security vulnerability reported. & {}\\
%           c. & Presence of vulnerability in PR/commits (not linked to external dependencies) & {} \\
%         % & L  & Time taken to detect vulnerabilities in pull requests \\
%         % &  & T  & Number of vulnerable commits processed over time \\
%         % &  & E & Efficiency of security checks on pull requests \\
%         \midrule
%         \textbf{2.} & \textbf{Security vulnerability in artifact -- use of vulnerable dependencies} & Assesses if vulnerable dependencies are introduced into the artifact\\
%         a. & Average length of time before fix & {} \\
%         b. & Severity levels of package’s reported vulnerability & {}  \\
%         c. &  Number of Repos/Projects that has a vulnerable dependency .& {} \\
%         d. & Average number of vulnerable dependencies/project. & {}  \\
%         e. & Average number of projects with reported vulnerable dependencies& {} \\
%         % & L  & Latency in detecting dependency vulnerabilities \\
%         % &  & T  & Number of dependencies checked over time \\
%         % &  & E & Efficiency of scanning vulnerable dependencies \\
%         \midrule
%         \textbf{3.} & \textbf{Use of ecosystem code scanning and security analysis features} & Evaluates usage of ecosystem's security tools for code scanning\\
%         a. & Status of dependabot alerts (for dependencies) & {}  \\
%          b. &  Status of Secret sharing/Validity Checks. & {}  \\
%          c. &  Code scanning and Vulnerability alerts & {}  \\ 
%        d. &  Push Protection Status & {} \\
%         % & L  & Time to complete a code scan \\
%         % &  & T  & Number of scans performed per time unit \\
%         % &  & E & Effectiveness of scanning tools \\
%         \midrule
%         \textbf{4.} & \textbf{Use of ecosystem integrity guarantees} & Examines use of ecosystem integrity features (e.g., code signing) \\
%          a. & Average Number of Projects with an integrity guarantee. & {}  \\
%          % L & {} & {} \\
%          %  L & {} & {} \\
%         % & L  & Time to apply integrity checks \\
%         % &  & T  & Number of integrity verifications done over time \\
%         % &  & E & Effectiveness of integrity tools \\
%         \midrule
%        \textbf{5.} & \textbf{Use of branch protection} & Checks if branch protection is enforced to prevent unauthorized changes\\
%          a. & Average Number of protected branch per project & {} \\
%          b. & Number of Projects with Protected branch  & {}\\
%           % L & {} & {} \\
%         % & L  & Time taken to apply branch protection \\
%         % &  & T  & Number of branches protected per unit of time \\
%         % &  & E & Efficiency of branch protection mechanisms \\
%         \midrule
%         \textbf{6.} & \textbf{Use of security policies and vulnerability reporting} & Determines if project has security policies and reporting mechanisms\\
%          a. & status of private vulnerability reporting, or security policy & {} \\
%          % L & {} & {} \\
%          %  L & {} & {} \\
%         % & L  & Time taken to report vulnerabilities \\
%         % &  & T  & Number of policies or reports handled \\
%         % &  & E & Clarity and effectiveness of security policies \\
%         \midrule
%         \textbf{7.} & \textbf{Use of automated workflows} & Assesses use of automation in workflows to enforce security.\\
%         a. & Average Number of Projects with Automated workflow & {}\\
%          % L & {} & {} \\
%          %  L & {} & {} \\
%         \bottomrule
% 		\end{tabular}
% 		\label{tab:signal_evaluation}
% 	\end{table*}
% }
%\arraystretch{1.5}
% \KC{TODOS;
% 1. Intro and background
% 2. add disclaimers for what work did and did not do.
% 3. Table caption and refs
% }
\begin{table*}[!t]
\centering
\caption{
    % Proposed security metrics and evaluation methods. Metric categories in bolded fonts are derived from recommendations from security recommendations from NIST, SLSA, and CNCF. Sub-metrics provide means of evaluating the proposed metrics. We also cite potential security case study that warrants inclusion of these metrics.
    Proposed security signals.
    Bolded signal categories are derived from security recommendations (e.g, NIST, CNCF, etc).
    \JD{Next sentence says `sub-metrics', which doesn't make sense without reference to appendix where we actually define them}
    % Evaluation metrics ~\cref{tab:signal_evaluation} offer ways to evaluate the bolded Signals, and relevant security case studies and or related works are cited to justify their inclusion.
      The proposed evaluation metrics in~\cref{tab:signal_evaluation} offer ways to evaluate the signals below.
    % We have categorized proposed security signals, and their descriptions and metrics are provided for evaluation purposes.
    \JD{Refer to the expanded version in the appendix}
    \JD{Put the references for the top-level signals into this table as well so things look less naked --- eg so [51,80,81] would show up for item 1. Also, in the appendix version, why are there no references for security signal 3 a-d?}
}
\normalsize
\small
\scriptsize
\begin{tabular}{p{0.01\linewidth}p{0.39\linewidth}p{0.50\linewidth}}
% p{0.13\linewidth}
% \textbf{Potential Case Study Use}
    \toprule
   \textbf{S/N.} &\textbf{Proposed Signals \& Analysis Metrics} & \textbf{Description} \\
\toprule
\textbf{} & \textbf{\textit{\ul{SECURITY SIGNALS}}} &  \\
%\hdashline[1.5pt/5pt]
 {} & {} & {} \\

\textbf{1.} & \textbf{Security vulnerability in artifact -- Pull Requests/Commits ~\cite{boughton_decomposing_2024, shukla_vulnerability_detection, gonzalez_anomalicious_2021}} & Measures vulnerabilities introduced through pull requests or commits. Introduced either by the user or to a project owned by the user. \\
%\hdashline[1.5pt/5pt]
% a. & Time to fix/close security vulnerabilities of various severity levels~\cite{boughton_decomposing_2024}& Time taken to address vulnerabilities detected in pull requests or commits.\\
% %\hdashline[1.5pt/5pt]
% b. & Severity levels of security vulnerability reported~\cite{shukla_vulnerability_detection} & Evaluates the criticality of reported vulnerabilities (low, medium, high), for user's projects.\\
% %\hdashline[1.5pt/5pt]
% c. & Presence of vulnerability in PR/commits (not linked to external dependencies)~\cite{gonzalez_anomalicious_2021} & Measures severity of vulnerabilities that stem from user's direct contributions. \\
% d. & Presence of vulnerability in PR/commits (not linked to external dependencies) & Measures whether vulnerabilities stem from direct contributions rather than external sources. \\
\midrule
\textbf{2.} & \textbf{Security vulnerability in artifact -- use of vulnerable dependencies ~\cite{boughton_decomposing_2024, shukla_vulnerability_detection}} & Assesses the use and introduction of vulnerable dependencies into the artifact. \\
%\hdashline[1.5pt/5pt]
% a. & Length of time before fix~\cite{boughton_decomposing_2024} & Time taken to resolve vulnerable dependencies, after they have been detected (or publicized).\\
% %\hdashline[1.5pt/5pt]
% b. & Severity levels of package’s reported vulnerability~\cite{shukla_vulnerability_detection} & Tracks severity of vulnerabilities in dependencies.\\
% %\hdashline[1.5pt/5pt]
% c. & Number of Repos/Projects that have a vulnerable dependency & Total number of projects affected by vulnerable dependencies as a percentage of users total projects.\\
% %\hdashline[1.5pt/5pt]
% d. & Number of vulnerable dependencies/project & Assesses how widespread vulnerable dependencies are within each project. \\
% %\hdashline[1.5pt/5pt]
% e. & Number of projects with reported vulnerable dependencies & Measures the overall exposure of projects to vulnerable dependencies. \\
\midrule
\textbf{3.} & \textbf{Use of ecosystem code scanning and security analysis features\cite{fischer2023effectiveness}} & Evaluates usage of ecosystem's security tools for code scanning. \\
% & Potentially stops the use of exposed user secrets ~\cref{colonial pipeline} 
%\hdashline[1.5pt/5pt]
% a. & Status of dependabot alerts (for dependencies) & Monitors if security alerts for dependencies are being addressed.\\
% %\hdashline[1.5pt/5pt]
% b. & Status of Secret sharing/Validity Checks & Evaluates the management of secret-sharing mechanisms and validity checks.\\
% %\hdashline[1.5pt/5pt]
% c. & Code scanning and Vulnerability alerts & Assesses if security scanning tools are actively used and vulnerability alerts managed. \\ 
% %\hdashline[1.5pt/5pt]
% d. & Push Protection Status & Checks if protection features are used to block pushes with exposed secrets (e.g., unscanned code). \\
\midrule
\textbf{4.} & \textbf{Use of ecosystem integrity guarantees~\cite{schorlemmer_signing_2024}} & Examines use of ecosystem integrity features (e.g., code signing). \\
%\hdashline[1.5pt/5pt]
% a. & Number of Projects with an integrity guarantee~\cite{schorlemmer_signing_2024} & Measures how many projects are secured with integrity verification features such as code signing. \\
\midrule
\textbf{5.} & \textbf{Use of branch protection~\cite{Scorecard,zahan2023openssf_snp}} & Checks if branch protection is enforced to prevent unauthorized changes. \\
%\hdashline[1.5pt/5pt]
% a. & Number of protected branches per project & Evaluates how many branches within each project are safeguarded against direct commits. \\
% %\hdashline[1.5pt/5pt]
% b. & Number of Projects with Protected branches~\cite{Scorecard,zahan_openssf_2023} & Tracks how many projects enforce branch protection. \\
\midrule
\textbf{6.} & \textbf{Use of security policies and vulnerability reporting~\cite{Scorecard}} & Determines if the project has security policies and reporting mechanisms. \\
%\hdashline[1.5pt/5pt]
% a. & Status of private vulnerability reporting, or security policy~\cite{Scorecard} & Checks if private vulnerability reporting channels and security policies are established and functional. \\
\midrule
\textbf{7.} & \textbf{Use of automated workflows~\cite{Scorecard}} & Assesses use of~\cite{Scorecard} automation in workflows to enforce security.\\
%\hdashline[1.5pt/5pt]
% a. & Number of Projects with Automated workflows~\cite{Scorecard} & Measures how many user's projects use automated workflows for security enforcement, such as auto-deployments or auto-tests. \\
\midrule
\midrule
\textbf{} & \textbf{\textit{\ul{REPUTATION WEIGHTAGE SIGNALS}}} &  \\
%\hdashline[1.5pt/5pt]
 {} & {} & {} \\
% \midrule
\textbf{W1.} & \textbf{Package Usage\cite{boysel_no_nodate}} & Weighs the utility of the potential contributor's owned projects \\
%\hdashline[1.5pt/5pt]
 % {a.} & {Number of downloads/stars/forks} & {Weighs the potential contributor's ownership of useful projects to the ecosystem.} \\
 \midrule
\textbf{W2.} & \textbf{Community Tenure \cite{boughton_decomposing_2024}} & Weighs the length of the contributor's belonging to the ecosystem  \\
%\hdashline[1.5pt/5pt]
 % {a.} & {Length of time contributing to project } & {Weighs how much time user has been a contributor to other projects.} \\
 %  {b.} & {Length of time owning account} & {Weighs how long user has actually owned an account}
 %  \\
   % {c.} & {Contributory Strength } & {Weighs the strength of contributions to other projects by lines of code, issues, pull requests}
   % \\
\midrule
\textbf{W3.} & \textbf{Centrality Score\cite{hamer_trusting_2025}} & Weighs the degree of connections of the potential contributor to other actors in the ecosystem. \\
%\hdashline[1.5pt/5pt]
 % {a.} & {Connections to other Actors\cite{hamer_trusting_2025}} & {Weighs a potential contributor's network of interactions/contributory activities.} \\
 %  {b.} & {Time to form connections} & {Length of time taken to form the connections in 'a' above.} \\
\bottomrule
\end{tabular}
\label{tab:signal_evaluation2}
\end{table*}
}
